LOQA: Learning with Opponent Q-Learning Awareness

In various real-world scenarios, interactions among agents often resemble the dynamics of general-sum games, where each agent strives to optimize its own utility. Despite the ubiquitous relevance of such settings, decentralized machine learning algorithms have struggled to find equilibria that maximize individual utility while preserving social welfare. In this paper we introduce Learning with Opponent Q-Learning Awareness (LOQA), a novel, decentralized reinforcement learning algorithm tailored to optimizing an agent's individual utility while fostering cooperation among adversaries in partially competitive environments. LOQA assumes the opponent samples actions proportionally to their action-value function Q. Experimental results demonstrate the effectiveness of LOQA at achieving state-of-the-art performance in benchmark scenarios such as the Iterated Prisoner's Dilemma and the Coin Game. LOQA achieves these outcomes with a significantly reduced computational footprint, making it a promising approach for practical multi-agent applications.

==> new_intro.tex <==
\section{Introduction}

What happens if each of us delegate all of our decision makings to RL agents that act on our behalf and are optimized to maximize our return? This is an important question as autonomous agents are already being integrated into our society. They are making decisions for us \cite{rl-in-finance, rl-in-healthcare, rl-in-medical-imaging}, simulating policy proposals for climate change negotiations \cite{zhang2022ai} and driving on behalf of their owner. To answer this, extrapolating current research indicates a potentially concerning scenario: countries could fail to reach climate deals, research labs might not share their tools with other research laboratories, and farmers may exploit shared water resources for their own plant growth. The reason behind these gloomy predictions is that we have substantial evidence that current naive MARL agents fail to solve social dilemmas which severely limits their practicality. 

Naive MARL agents cannot reach reciprocation-based cooperation even in simple matrix environments. Two naive RL agents optimizing their return in an environment as simple as Iterated Prisoner's Dilemma (IPD) converge to always defect(AD) policies. They miss the tit-for-tat(TFT) solution which has a higher return than the AD and enables conditional cooperation. Although optimizing agents for the shared reward looks like a simple fix it leads to exploitable agents that always cooperate(AC). Reciprocation is key. Therefore, algorithms that enable emergence of reciprocation hold tremendous theoretical and practical value. 

 Naive RL algorithms assume the opponents' policies are static in each policy update. By not accounting for the opponents' optimizing their return the naive RL agent misses the potential to shape the learning of the opponents. This shaping is possible because The outcome of each opponent is determined not only by their own actions but also of the agent \cite{vonNeumann1928}. LOLA \cite{Foerster2018a}, POLA, M-FOS, Good Shepherd, and Meta-Value enable emergent reciprocation by shaping the opponents' learning \todo{cite these papers}. 

However, the existing algorithms don't scale. LOLA and POLA differentiate through an assumed naive gradient step of the opponent by explicit computations graphs of the opponent's optimization. For neural network policies that need many steps to optimize their return it means they need thousands of explicit optimization step roll-outs. Next, the agent differentiates through this complex computational graph, which leads to huge computational and memory costs and also higher order-gradients. M-FOS, Good-Shepherd, Meta-Value, and others(\todo{which others}) shape the opponent by constructing a meta-game in the space of agent policies. They define the problem as a meta-state over the product space of policies of the agent and opponent, and learns a meta-policy that maps from the meta-state to the agent's updated policy. Therefore they need to learn the dynamics of multiple agents simultaneously being optimized to guide the optimization of the opponent afterwards. This is very challenging in Deep RL as learning the optimization dynamics of multiple neural network policies is complex, hard, and sample inefficient. While, in fully competitive and fully cooperative large scale environments RL algorithms have super-human performance, the state-of-the-art in solving social dilemmas is solving the 3x3 coin game. This shows the need for faster algorithms with less computational and memory requirements. In other words, more scalable algorithms.  


%The dynamics of interactions between agents in the real world almost always have a mix of competitive cooperative elements. For example, Each individual country benefits from more carbon emission, but it also needs to maintain a healthy climate condition.

%However, these scenarios are different from the main focus of the DeepRL research - the fully competitive or fully cooperative - environments as the dynamics of interactions between agents in the real world almost always contains a mix of competition and cooperation - social dilemma. For example, Countries wants to compete by producing more which induces more carbon emission but they share the same climate and should keep the living conditions stable. The situations in which an environment is fully cooperative or fully competitive are limited and mostly preserved for video games. While Deep RL agents achieve human level performance on large scale fully cooperative or fully competitive games (TODO cite skycraft, dota, chess), they fail at solving the simplest environments that contain a social dilemma. 

In this paper we introduce Q-value Shaping (QS). QS is an scalable algorithm that side-steps both building explicit iterative computational graphs of optimization steps or learning the meta-state dynamics altogether by making a key observation. The optimization step of each opponent is shaped by that opponent's return. As the return of every opponent is dependent on the agent actions in a multi agent environment, the agent can shape the optimization of opponents, by shaping their return.  Explicitly, each opponent is assumed to optimize its policy to choose the action with the highest action-value. This action-value is differentiable w.r.t the agent parameters. QS build a steerable approximated policy of the opponent by a softmax over its action-values which is close to (TODO: should mention sac). QS shapes the opponent's return, and the optimization step of the opponent will be shaped indirectly as a result. Therefore, QS does not involve neither building complex optimization computational graphs nor second order gradients which leads to significant computational efficiency. 

We experiment with QS on IPD to show its capability to solve simple environments and on the coin game to show its superior scalability as solving the 3x3 coin game is the state of the art in this subfield. We showcase the scalability of QS in two directions: 1) QS reached reciprocation-based cooperation 30 times faster than POLA (SOTA) on 3x3 coin game. 2) QS reaches strong reciprocation-based cooperation in 7x7 coin game where POLA fails and just learns always defect strategies. We summarize our contributions as follows:
\begin{enumerate}[leftmargin=3pt]
\item We propose Q-value Shaping(QS) which shapes opponent's learning via shaping its action-values.
\item QS does not involve computing opponent optimization steps, let alone differentiating through the constructed computational graph, high-order gradients, and learning optimization dynamics of multiple agents all of which hindered the scalability of previous methods significantly.
\item We show QS reaches the same performance the previous SOAT algorithm, POLA,  on the SOTA benchmark, 3x3 coin game 30 times faster using the same hardware setup. Also, QS solves the 7x7 coin game where POLA fails.
\end{enumerate}

==> new_intro_1.tex <==
\section{Introduction}

What happens if we delegate all of our decision making processes to RL agents that act on our behalf to maximize our return? Current research indicates that countries could not reach climate deals, research labs would not share their tools with other research laboratories, farmers would exploit their water resources for their own plant growth. This is because naive MARL agents fail to solve social dilems. 
Failing to solve social dilemmas severely limits the practicality of RL agents. However, the current algorithms that navigate social dilemmas are limited in their scalability.

Autonomous agents are being integrated in the society. To name a few, they are used in decision making processes(TODO), simulating policy proposals for climate change negotiations and even driving on behalf of their owner(TODO cite tiyanio). However, these scenarios are different from the main focus of the DeepRL research - the Fully Competitive or Fully Cooperative - environments as the dynamics of interactions between agents in the real world almost always contains a mix of competition and cooperation - social dilemma. For example, Countries wants to compete by producing more which induces more carbon emission but they share the same climate and should keep the living conditions stable. The situations in which an environment is fully cooperative or fully competitive are limited and mostly preserved for video games. While Deep RL agents achieve human level performance on large scale fully cooperative or fully competitive games (TODO cite skycraft, dota, chess), they fail at solving the simplest environments that contain a social dilemma. 

Optimizing two RL agents in an environment as simple as Iterated Prisoner's Dilemma leads to policies that always defect. Naive RL agents miss the tit-for-tat(TFT) solution as they fail to form a reciprocity-based cooperation. While both of Always Defect and TFT are Nash Equilibriums of the IPD game, the naive solutions leads to the one with the lowest return(TODO: Is this the lowest). Sharing rewards of the agents looks like a simple fix until we realize that it leads to exploitable agents that always cooperate and the key is being reciprocation-based. As naive agents fail to build reciprocation-based cooperation they change to always defecting to increase their return. This paints a gloomy future where these agents are deployed in the real world facing the large scale and complex dynamics of social dilemmas. How this reciprocation emerges is therefore a key question which has tremendous theoretical and practical value. 

In each Naive RL policy update, the agents assume the other agents are static. This stationary assumption about the environment is deeply rooted in current RL algorithms. However, when training multiple agents simultaneously, every agent's policy is changing at the same time. They do not account for the fact that the other agents are also in their optimization process. Taking this fact into account unlocks a huge potential of shaping other agents' learning process as the outcome of each agent is determined not only by their own actions but also those of other players \cite{vonNeumann1928}.

There are algorithms that take the opponent learning process into account. But, they have strict scalability problems. LOLA and POLA take the opponent learning step into account by differentiating through an assumed naive gradient step of the opponent.  They build explicit computations graphs of the opponent's assumed update. However, for policies that need many update steps to optimize their return it means they need thousands of explicit roll-out of the optimization step. Next, the agent should differentiate through this huge computational graph, which leads to huge computational and memory costs and higher order-gradients. M-FOS, Good-Shepherd, Meta-Value, and others(TODO) shape the opponent by constructing a meta-game in the space of agent policies. They define the problem as a meta-state over the product space of policies of the agent and opponent, and learns a meta-policy that maps from the meta-state to the agent's updated policy. (TODO: best argument for this being non-scalable) Therefore they need to learn the dynamics of multiple agents simultaneously being optimized to guide the optimization of the opponent afterwards. This is very challenging in Deep RL as Learning the optimization dynamics of multiple neural network policies is complex, hard, and sample inefficient.


In this paper we introduce Q-value Shaping (QS). QS side-steps building explicit iterative computational graphs of optimization steps and learning the meta-state dynamics altogether by making a key observation. The optimization step of each opponent is shaped by that opponent's return. As the return of every opponent is dependent on the agent actions in a multi agent environment, the agent can shape the optimization of opponents, by shaping their return.  Explicitly, each opponent is assumed to optimize its policy to choose the action with the highest action-value. This action-value is differentiable w.r.t the agent parameters. QS build a steerable approximated policy of the opponent by a softmax over its action-values which is close to (TODO: should mention sac). QS shapes the opponent's return, and the optimization step of the opponent will be shaped indirectly as a result. Therefore, QS does not involve neither building complex optimization computational graphs nor second order gradients which leads to significant computational efficiency. 

We experiment with QS on IPD to show its capability to solve simple environments and on the coin game to show its superior scalability as solving the 3x3 coin game is the state of the art in this subfeild. We showcase the scalability of QS in two directions: 1) QS reached reciprocation-based cooperation 30 times faster than POLA (SOTA) on 3x3 coin game. 2) QS reaches strong reciprocation-based cooperation in 7x7 coin game where POLA fails and just learns always defect strategies. 

We summarize our contributions as follows:
\begin{itemize}
\item We propose QS, that shapes opponent's optimization by shaping the opponent's action-values
\item QS does not involve computing opponent optimization steps, let alone differentiating through the constructed computational graph, high-order gradients, and learning optimization dynamics of multiple agents all of which hindered the scalability of previous methods significantly.
\item We show QS reaches the same performance the previous SOAT algorithm, POLA,  on the SOTA benchmark, 3x3 coin game 30 times faster using the same hardware setup. Also, QS solves the 7x7 coin game where POLA fails.
\end{itemize}

==> old_intro.tex <==
\section{Introduction}

A major difficulty in reinforcement learning (RL) and multi-agent reinforcement learning (MARL) is the non-stationary nature of the environment, where the outcome of each agent is determined not only by their own actions but also those of other players \cite{vonNeumann1928}. This difficulty often results in the failure of traditional algorithms converging to desirable solutions. In the context of general-sum games, independent RL agents often converge to sub-optimal solutions in the Pareto sense, when each of them seeks to optimize their own utility \cite{Foerster2018a}. This situation draws parallels with many real-world scenarios, in which individuals pursuing their own selfish interests leads them to a worse outcome than cooperating with others. Thus one of the objectives of MARL research must be to develop decentralized agents that are able to cooperate while avoiding being exploited in partially competitive settings. We call this reciprocity-based cooperation.

Previous work has resulted in algorithms that train reciprocity-based cooperative agents by differentiating through the opponent's learning step \citep{Foerster2018a, Letcher2021, Zhao2022, Willi2022} or by modeling opponent shaping as a meta-game in the space of agent policies \citep{Alshedivat2018, Kim2021, Lu2022, Cooijmans2023}. However, both of these approaches have important drawbacks with respect to computational efficiency. On one hand, differentiating through even just a few of the opponent’s learning steps, can only be done sequentially and requires building large computation graphs. This is computationally costly when dealing with complex opponent policies. On the other hand, meta-learning  defines the problem as a meta-state over the product space of policies of the agent and opponent, and learns a meta-policy that maps from the meta-state to the agent's updated policy. The complexity of the problem then scales with the policy parameterization which is usually a neural network with many parameters.

In this paper we introduce Learning with Opponent Q-Learning Awareness (LOQA), which stands because it avoids computing gradients w.r.t. optimization steps or learning the dynamics of a meta-game, resulting in significantly improved computational efficiency. LOQA performs opponent shaping by assuming that the opponent's behavior is guided by an internal action-value function $Q$. This assumption allows LOQA agents to build a model of the opponent policy that can be shaped by influencing its returns for different actions. Controlling the return by differentiating through stochastic objectives is a key idea in RL and can be done using the REINFORCE estimator \cite{Williams1992}.
